BotNet: A Simulator for Studying the Effects of Accurate Communication Models on Multi-agent and Swarm Control

Decentralized control in multi-robot systems is dependent on accurate and reliable communication between agents. Important communication factors, such as latency and packet delivery ratio, are strong functions of the number of agents in the network. Findings from studies of mobile and high node-count radio-frequency (RF) mesh networks have only been transferred to the domain of multi-robot systems to a limited extent, and typical multi-agent robotic simulators often depend on simple propagation models that do not reflect the behavior of realistic RF networks. In this paper, we present a new open source swarm robotics simulator, BotNet, with an embedded standards-compliant time-synchronized channel hopping (6TiSCH) RF mesh network simulator. Using this simulator we show how more accurate communications models can limit even simple multi-robot control tasks such as flocking and formation control, with agent counts ranging from 10 up to 2500 agents. The experimental results are used to motivate changes to the inter-robot communication propagation models and other networking components currently used in practice in order to bridge the sim-to-real gap.

==> _appendics.tex <==
% \section*{Appendix}

% \subsection{Flocking with Minimal Scheduling Function}
% The 6TiSCH simulator includes a minimal schedule function by default, which is designed for stationary nodes.
% These experiments are a supplement to those shown in \sect{sec:exp}, specifically \fig{fig:flock1}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.9\linewidth]{figures/MSF_flock.pdf}
%     \caption{
%     Median and standard deviation flocking velocity for different potential control connectivity radii (10 trials per configuration, 10 agents per trial, MSF). 
%     Average velocities close to zero generally indicate that the flock fails to follow the leader agent. 
%     The results show that using more realistic propagation models in the networking simulation stack sets bounds on the potential control flocking radius; at higher radii, agents lose connection from the leader and potentially their neighbors (depending on collision radius).
%     }
%     \label{fig:flock_msf}
% \end{figure}
